Resource Allocation in Multi-armed Bandit Exploration: Overcoming Sublinear Scaling with Adaptive Parallelism

We study exploration in stochastic multi-armed bandits when we have access to a divisible resource that can be allocated in varying amounts to arm pulls. We focus in particular on the allocation of distributed computing resources, where we may obtain results faster by allocating more resources per pull, but might have reduced throughput due to nonlinear scaling. For example, in simulation-based scientific studies, an expensive simulation can be sped up by running it on multiple cores. This speed-up however, is partly offset by the communication among cores, which results in lower throughput than if fewer cores were allocated per trial to run more trials in parallel. In this paper, we explore these trade-offs in two settings. First, in a fixed confidence setting, we need to find the best arm with a given target success probability as quickly as possible. We propose an algorithm which trades off between information accumulation and throughput and show that the time taken can be upper bounded by the solution of a dynamic program whose inputs are the gaps between the sub-optimal and optimal arms. We also prove a matching hardness result. Second, we present an algorithm for a fixed deadline setting, where we are given a time deadline and need to maximize the probability of finding the best arm. We corroborate our theoretical insights with simulation experiments that show that the algorithms consistently match or outperform baseline algorithms on a variety of problem instances.

==> figs__Kirthevasan_Kandasamy_s_conflicted_copy_2021-02-04_.tex <==
\newcommand{\insertFigSettingIllus}{%
\begin{figure}
% \centering
\includegraphics[width=3.0in]{figures/sublinear_scaling.png}
\caption{\small
An illustration of our  setting. An algorithm has a divisible resource (green circle) that can be split up to generate samples from the arms. Each pull takes \emph{time} to complete, where the time taken is a decreasing function of the number of resources used. Allocating more resources results in faster results, but at the cost of decreased throughput. When a pull completes, the resources used are freed and can be reallocated to new pulls. In this example, the pull using half the resources (red semicircle) to pull arm 1 (red) finishes before the pulls using a quarter of the resources (quarter circles). When the pull completes, half of the resources are available (green semicircle) and are reallocated to generate three new samples from arms 1 and 2.
\label{fig:settingillus}
}
\end{figure}[ht]
}

% fixed the positioning issue - Brijen

\newcommand{\insertFigDistParIllus}{%
\begin{figure*}
\centering     %%% not \center
\includegraphics[width=6.0in]{figures/distributed_bandits_splash.png}
\vspace{-0.1in}
\caption{\small{\emph{Left:} A sequential strategy will allocate all
resources to individual jobs/arm pulls.
This 
enables the algorithm to obtain information about individual pulls sooner for replanning; after
pulling all arms twice, it is able to eliminate the green arm.
However, this reduces throughput due to non-ideal scaling, and can take a long time.
\emph{Middle:} A highly-parallel strategy with fixed batch size will have higher throughput but may
evaluate the poor arms too many times and take longer to eliminate them.
\emph{Right:} Our algorithm for the fixed confidence
setting adaptively
manages parallelism during execution based on the scaling function and/or task progress.
In this figure, the green arm is eliminated early, and then throughput is increased for the
remaining $2$ arms which may be harder to distinguish.
While the setting permits allocating the resources ``asynchronously'' (see
Fig.~\ref{fig:settingillus}), we show that an algorithm which operates synchronously, but
chooses the amount of parallelism adaptively is minimax optimal for this problem.
}
% \kkcomment{The titles for each of the three figures is a bit strange. Can we change them?}
\label{fig:tradeoffillus}
}
% \vspace{-0.15in}
\insertfigcaptionspacing
\end{figure*}
}

\newcommand{\insertFigFixedConf}{%
\begin{figure*}[h]
\includegraphics[width=\linewidth]{figures/neurips_2020_plots_conf.png}\label{fig:fixed_conf_experiments}
\vspace{-0.30in}
\caption{\small{\textbf{Fixed confidence synthetic results:} We vary the first gap $\Delta_2$ from $0.01$ to $0.5$ for $q \in \{0.1, 0.25, 0.5, 0.9\}$. A higher $\Delta_2^{-2}$ (right side) implies the problem is harder to solve as more arm pulls will be needed to separate the confidence bounds of the best arm from the rest. We present the mean and standard error across $10$ runs for all experiments. We observe that Algorithm~\ref{alg:fixed_confidence} (APR) is able to trade off between throughput and information accumulation effectively in most cases without additional hyperparameters, consistently performing near the best algorithms for each problem. The baseline algorithms perform well when their level of parallelism is well-suited to the scaling and $\Delta_i$ values of the problem, but are inconsistent across problems.\vspace{-0.2in}
}}
\vspace{0.1in}
\end{figure*}
}

\newcommand{\insertFigFixedDeadline}{%
\begin{figure*}[h]
\centering     %%% not \center
\subfigure{\label{fig:c1h}\includegraphics[width=40mm]{figures/fixed_budget/exp_budget_acc_09.png}}
\subfigure{\label{fig:c1f}\includegraphics[width=40mm]{figures/fixed_budget/exp_budget_acc_05.png}}
\subfigure{\label{fig:c1d}\includegraphics[width=40mm]{figures/fixed_budget/exp_budget_acc_025.png}}
\subfigure{\label{fig:c1b}\includegraphics[width=40mm]{figures/fixed_budget/exp_budget_acc_01.png}}
\vspace{-0.2in}

\subfigure{\label{fig:c1g}\includegraphics[width=40mm]{figures/fixed_budget/exp_budget_x_09.png}}
\subfigure{\label{fig:c1e}\includegraphics[width=40mm]{figures/fixed_budget/exp_budget_x_05.png}}
\subfigure{\label{fig:c1c}\includegraphics[width=40mm]{figures/fixed_budget/exp_budget_x_025.png}}
\subfigure{\label{fig:c1a}\includegraphics[width=40mm]{figures/fixed_budget/exp_budget_x_01.png}}
\vspace{-0.1in}
\caption{\small{\textbf{Fixed deadline synthetic results:} We vary the time budget for $q \in \{0.1,
0.25, 0.5, 0.9\}$, running for $10$ runs each and presenting the mean and standard error. We find
that SSH (red) consistently outperforms SH (green) and UCB-E (blue).
This difference is large when the scaling is poor ($q$ is small) as
SH does not pull each arm a sufficient number of times before each stage ends, 
and the cost of allocating all resources to individual pulls prevents UCB-E from
making progress in comparable time.
In contrast, \scsh{} does well because it prioritizes high throughput when the scaling is poor.
% This throughput reduction is analogous to
% sublinear scaling in parallel computing due to communication and synchronization costs.
% For worse
% scaling functions, the cost of allocating all resources to individual pulls prevents UCB-E from
% making progress in comparable time. 
When $q=0.1$, SH and UCB-E perform poorly whereas when $q\geq 0.5$, \scsh{} has similar throughput
as SH, resulting in similar performance.}\label{fig:fixed_budget_exps}}
% \vspace{-0.1in}
\end{figure*}
}

